Learning Task-General Representations with Generative Neuro-Symbolic Modeling

People can learn rich, general-purpose conceptual representations from only raw perceptual inputs. Current machine learning approaches fall well short of these human standards, although different modeling traditions often have complementary strengths. Symbolic models can capture the compositional and causal knowledge that enables flexible generalization, but they struggle to learn from raw inputs, relying on strong abstractions and simplifying assumptions. Neural network models can learn directly from raw data, but they struggle to capture compositional and causal structure and typically must retrain to tackle new tasks. We bring together these two traditions to learn generative models of concepts that capture rich compositional and causal structure, while learning from raw data. We develop a generative neuro-symbolic (GNS) model of handwritten character concepts that uses the control flow of a probabilistic program, coupled with symbolic stroke primitives and a symbolic image renderer, to represent the causal and compositional processes by which characters are formed. The distributions of parts (strokes), and correlations between parts, are modeled with neural network subroutines, allowing the model to learn directly from raw data and express nonparametric statistical relationships. We apply our model to the Omniglot challenge of human-level concept learning, using a background set of alphabets to learn an expressive prior distribution over character drawings. In a subsequent evaluation, our GNS model uses probabilistic inference to learn rich conceptual representations from a single training image that generalize to 4 unique tasks, succeeding where previous work has fallen short.

==> figures/type_model.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\hsize]{images/type_model.pdf}
	\caption{Neuro-symbolic type prior $P(\psi)$.
	Our type prior produces character samples one stroke at a time, using an image canvas $C$ as memory state.
	At each time step, the current canvas $C$ is fed to procedure \texttt{GeneratePart}, which produces a stroke sample.
	The canvas is first processed by the \textit{location model}, a CNN-MLP architecture that returns a Gaussian mixture model (GMM) distribution for the starting location $y$ of the next stroke. 
	The location is then sampled and passed along with $C$ to the \textit{stroke model}. 
	The stroke model processes $C$ with a CNN and feeds the embedding to an LSTM with attention. 
	The LSTM samples a stroke trajectory $x$ sequentially one offset at a time using GMM outputs.
	The sampled stroke is passed to a symbolic renderer, and the updated image canvas is then processed by a \textit{termination model} that decides whether to continue the character sample.
	}
    \label{fig:type_model}
\end{figure}
